The Blessings of Multiple Treatments and Outcomes in Treatment Effect Estimation

Assessing causal effects in the presence of unobserved confounding is a challenging problem. Existing studies leveraged proxy variables or multiple treatments to adjust for the confounding bias. In particular, the latter approach attributes the impact on a single outcome to multiple treatments, allowing estimating latent variables for confounding control. Nevertheless, these methods primarily focus on a single outcome, whereas in many real-world scenarios, there is greater interest in studying the effects on multiple outcomes. Besides, these outcomes are often coupled with multiple treatments. Examples include the intensive care unit (ICU), where health providers evaluate the effectiveness of therapies on multiple health indicators. To accommodate these scenarios, we consider a new setting dubbed as multiple treatments and multiple outcomes. We then show that parallel studies of multiple outcomes involved in this setting can assist each other in causal identification, in the sense that we can exploit other treatments and outcomes as proxies for each treatment effect under study. We proceed with a causal discovery method that can effectively identify such proxies for causal estimation. The utility of our method is demonstrated in synthetic data and sepsis disease.

==> chap/Experiments.tex <==
\vspace{-0.2cm}
\section{Experiments}
\vspace{-0.1cm}
\label{sec.experiment}

In this section, we evaluate our method on synthetic data and a real-world application, \emph{i.e.}, treatment of sepsis disease.

\noindent\textbf{Compared baselines.} \emph{Independence test}: \textbf{i) Fisher} that Fisher’s Z conditional independence test ; \textbf{ii) Chisq} that Chi-squared conditional independence test; \textbf{iii) POP} that The Promises of Parallel Outcomes. \emph{Causal estimation}: \textbf{i) GPS} that used generalized propensity scores to estimate causal effects; \textbf{ii) TMLE} that used Targeted Maximum Likelihood Estimation to estimate causal effects; \textbf{iii) POP} that used multiple outcomes and linear structural equations to estimate causal effects; \textbf{iv) Deconf.} that used the deconfounding method to estimate causal effects; \textbf{v) S-Deconf.} that used the deconfounding method to estimate causal effects under shared confounders.

\noindent\textbf{Evaluation metrics.} For the hypothesis test, we use the $\mathrm{F}_1$-score, precision, and accuracy of identified causal edges, and ${\mathrm{F}}_{1}:=2\cdot{\frac{\mathrm{precision}\cdot\mathrm{recall}}{\mathrm{precision+recall}}}$. For the causal effect estimation, we report the causal Mean Squared Error (cMSE) of point treatment 0 and 1 That is, {\small $\mathrm{cMSE}:=(\mathbb{E}[Y^{1}-Y^{0}]-\hat{\mathbb{E}}[Y^{1}-Y^{0}])^2$}.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.7\textwidth]{Figure/exp_DAG.pdf}
    \caption{The underlying causal graph with observed variables marked blue. (a) Causal DAG for Synthetic Data. (b) Causal DAG predicted using proxies-based hypothesis testing method, where abbreviations are provided in the appendix.}
    \label{fig: exp_DAG}
\end{figure}

\vspace{-0.2cm}
\subsection{Synthetic study}
\vspace{-0.1cm}

\noindent\textbf{Data generation.} We consider five treatments $\{A_i\}_{i=1}^5$, four outcomes$\{Y_i\}_{i=1}^4$, and one unobserved confounder $U$\footnote{Please refer to the appendix for settings with more unobserved confounders.}. We use the following structural equations: $U\sim \operatorname{Uniform
}[-1,1]$, $A_i=g_i(U)+\epsilon_i$, with $g_i$ chosen from $\{linear,tanh,sin,cos,sigmoid\}$ and $\epsilon_i\sim N(0,1)$, and $\mathbf{Y}$ is a non-linear structure, namely
$Y_1 = 2\sin(1.4A_1+2A_3^2)+0.5A_2+A_2^2+U+\epsilon_1, Y_2 = -2\cos(1.8A_2)+1.5A_4^2+U+\epsilon_{2}, Y_3 = 0.7A_3^2+1.2A_4+U+\epsilon_{3}$, and $Y_4 = 1.6e^{-A_1+1}+2.3A_5^2+U+\epsilon_{4}$  with $\{\epsilon_i\}_{i=1}^4 \sim N(0,1)$.

\vspace{-0.2cm}
\subsubsection{Identify Proxies}
\vspace{-0.1cm}

\noindent\textbf{Implementation details.} The significant level $\alpha$ is set to 0.05.  For our method, the $A,W,Y$ are discretized by quantile, with bin numbers (resp.) setting to $I = 15, K = 8, L = 5$ for synthetic data. The asymptotic estimators in (2)-(3) are obtained by empirical probability mass functions. The sample size is set to $\{600,800,1000,1200,1400,1600\}$. To remove the effect of randomness, we repeat for $50$ replications.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.85\textwidth]{Figure/discover.pdf}
    \caption{Performance of our method and baselines under the setting of multi-treatments and multi-outcomes.}
    \label{fig:discover}
\end{figure}

\noindent\textbf{Causal discovery.} We use the proxy-based hypothesis test to recover the causal graph and report the results under different sample sizes.  Fig.~\ref{fig:discover} shows the performance of our method and baselines under the setting of multi-treatments and multi-outcomes. As we can see, our method
significantly outperforms the others on all metrics. First, it can be observed that the POP method with a similar multi-outcomes setting to ours achieves very low performance, which is attributed to their assumption that the structural equations are all linear, which is difficult to happen in reality. Second, Chisq testing tends to connect every edges, and it has a large Type I error. We speculate that this is caused by the highly nonlinear structural equations. Lastly, compared to Fisher's testing, we perform better and have less fluctuations since we exploit the information of the proxy (other treatments).

\vspace{-0.2cm}
\subsubsection{Causal effect estimation}
\vspace{-0.1cm}

\noindent\textbf{Implementation details.} We use the PMMR method \cite{mastouri2021proximal} to solute the nuisance function $h$ and $q$. And for $q$ we use the estimation formula based on kernel function approximation. We run each algorithm 20 times with sample size $600$ or $1, 200$ and calculate the mean causal-MSE of point treatments 0 and 1.
 

\noindent\textbf{Causal effect estimation.} We estimate the average causal effect of $A_2\to Y_2$, $A_4\to Y_3$, $(A_1,A_2)\to Y_1$, $(A_1,A_5)\to Y_4$ and report the results in Tab.~\ref{tab:synthetic}. As we can see, estimating nuisance functions using non-parametric methods significantly outperforms other baselines for causal effects, which demonstrate its effectiveness in estimating the causal effect with proxy variables. Notably, when we estimate the effect of $A_4\to Y_3$, since the structure function is linear on $A_4$, specifying the parameter method of the linear model will give better results. However, our experiments also verified that the S-Deconf. method using proxy variables achieves smaller bias than the often-criticized Deconf. method, which also proves the power of the proxy. Besides, POP assumed the structure function is linear and each treatment points to all outcomes, thus it obtain poor performance.

\noindent\textbf{Correct Proxy.} In Fig.~\ref{fig:Synthetic_study}(a), we show the performance of the three methods on 300 samples (small sample). We estimate the causal effect for 50 points in $[0,2.5]$ and then plot the figure. We find that the PMMR-KIPW method that uses the kernel function to approximate the indicator function will have a relatively large variance, but the mean is also close to the true value. The PMMR-DR method using both nuisance functions $h$ and $q$ obtain the best performance. In addition, in order to emphasize the importance of correct proxy, we change the structural equation of $Y_3$ to $Y_3 = 0.7A_3+1.2A_4+U+N(0,1)$. We use the S-Deconf. method to estimate causal effects. We find that despite the linearity of the structural equations, large MSEs can still be produced when proxies are misspecified.

\begin{table}[htbp]
  \centering
  \caption{C-MSE of PMMR-X and baseline methods i Synthetic study. Each method was replicated 20 times and evaluated test values of $\mathbb{E}[Y^{1}-Y^{0}]$ each replicate.}
   \scalebox{0.77}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{$A_2 \rightarrow Y_2$} & \multicolumn{2}{c|}{$A_4 \rightarrow  Y_3$} & \multicolumn{2}{c|}{$\left(A_1, A_2\right) \rightarrow Y_1$}& \multicolumn{2}{c}{$\left(A_1, A_5\right) \rightarrow Y_4$} \\
\cline{2-9}          & 600   & 1200  & 600   & 1200  & 600   & 1200  & 600   & 1200 \\
    \hline
    GPS   & $3.32_{\pm 5.80}$ & $1.72_{\pm 1.80}$ & $0.51_{\pm 0.67}$     & $0.21_{\pm 0.24}$ &   -    & - &   -    & - \\
    TMLE   & $2.79_{\pm 4.59}$ & $1.08_{\pm 1.10}$ & $0.40_{\pm0.39}$     & $0.29_{\pm 0.37}$ &   -    & - &   -    & - \\
    POP   & $6.02_{\pm 0.00}$ & $6.66_{\pm 1.40}$ & $1.47_{\pm 0.18}$     & $1.23_{\pm 0.62}$ &   -    & - &   -    & - \\
    Deconf.  & $5.44_{\pm 2.80}$ & $5.73_{\pm 2.26}$ & $0.10_{\pm 0.10}$  & $0.07_{\pm 0.12}$ & $0.92_{\pm 0.73}$  & $1.36_{\pm 0.71}$ & $12.81_{\pm 4.66}$ & $10.2_{\pm 4.00}$ \\
    S-Deconf. & $4.94_{\pm 0.89}$ & $4.78_{\pm 0.89}$ & $\mathbf{0.01_{\pm 0.01}}$ & $\mathbf{0.01_{\pm 0.01}}$ & $14.1_{\pm 35.9}$  & $5.59_{\pm 5.36}$ & $18.7_{\pm 1.65}$  & $18.8_{\pm 2.45}$   \\
    PMMR-OR     & $\mathbf{0.27_{\pm 0.35}}$ & $\mathbf{0.14_{\pm 0.24}}$ & $0.16_{\pm 0.16}$ & $0.08_{\pm 0.11}$ & $0.20_{\pm 0.25}$ & $0.10_{\pm 0.12}$ & $0.58_{\pm 0.40}$ & $\mathbf{0.05_{\pm 0.06}}$ \\
    PMMR-KIPW     & $0.68_{\pm 0.87}$ & $0.89_{\pm 1.85}$ & $0.57_{\pm 0.61}$ & $0.52_{\pm 0.62}$ & $0.32_{\pm 0.34}$ & $0.26_{\pm 0.36}$ & $0.55_{\pm 0.19}$ & $0.19_{\pm 0.20}$ \\
    PMMR-DR     & $0.59_{\pm 0.60}$ & $0.61_{\pm 0.74}$ & $0.15_{\pm 0.18}$ & $0.22_{\pm 0.40}$ & $\mathbf{0.15_{\pm 0.22}}$ & $\mathbf{0.09_{\pm 0.12}}$ & $\mathbf{0.18_{\pm 0.28}}$ & $0.24_{\pm 0.38}$ \\
    \hline
    \end{tabular}}
  \label{tab:synthetic}%
\end{table}%



\begin{figure}[htbp]
\begin{minipage}{.5\textwidth}
\label{fig:ate_300}
\centering
\includegraphics[width=0.7\linewidth]{Figure/ate_300.pdf}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\label{fig:proxy}
\centering
\includegraphics[width=0.7\linewidth]{Figure/proxy.pdf}
\end{minipage}
\caption{Left: ATE comparison with ground truth and different methods on $A_3\to Y_3$. The causal-mse of different methods for $a\in[0,2.5]$ with samples of 300; lower is better. Right: Comparing causal estimates for two cases of whether the proxies is correctly specified.}
\label{fig:Synthetic_study}
\end{figure}

\vspace{-0.2cm}
\subsection{Treatment of sepsis disease}
\vspace{-0.1cm}
In this section, we apply our method to estimate the causal effect of different treatments in sepsis disease.

\noindent\textbf{Data extraction.} We consider the Medical Information Mart for Intensive Care (MIMIC III) dataset \cite{johnson2016mimic}, which consists of electronic health records from patients in the Intensive Care Unit (ICU). From MIMIC III, we extract $1165$ patients for which there are three treatment options during their stays: Vancomycin, Morphine Sulfate, and Norepinephrine (all of which can be applied simultaneously). These treatments are common in the ICU and are often used to treat patients with sepsis. At the next moment, we extract three outcomes (blood count indexes): White blood cell count, Mean blood pressure, and Platelets.

\noindent\textbf{Implementation details.} For hypothesis testing,  the significant level $\alpha$ is set to 0.05, and the $A,W,Y$ are discretized by uniform, with bin numbers (resp.) setting to $I = 10, K = 6, L = 5$. For treatment effect

\noindent\textbf{Causal discovery.} We show the learned causal graph in Fig.~\ref{fig: exp_DAG}(b). As shown, the Vancomycin has a causal influence on the White blood cell count and Platelets, which well align the clinical findings \cite{rosini2015randomized,mohammadi2017vancomycin}.  Also, Fig.~\ref{fig: exp_DAG} shows that the prescription morphine can causally influences the Mean blood pressure, and Platelets without affecting white blood cell counts, which is consistent with the pharmacology side-effects of morphine found in \cite{anand2004effects,degrauwe2019influence,simons2006morphine}. In addition, we can also observe that the Norepinephrine has a causal effect on all blood count indexes, which is also found in \cite{gader1975effect,larsson1994norepinephrine,belin2023manually}.

\noindent\textbf{Causal effect estimation.} We estimate the average causal effect of $VAN\to WBC$, $NE\to MBP$, $MS\to PLT$ and report the results in Tab.~\ref{tab:real}. As we can see, the Vancomycin, used to control bacterial infections in septic patients, lowers white blood cell counts because of its bactericidal and anti-inflammatory properties. Besides, Norepinephrine, as a vasopressor, can increase blood pressure. Also, Tab.~\ref{tab:real} shows that Morphine has a negative effect on platelet counts. Our findings are consistent with the literature studying the effects of three drugs on blood count indexes \cite{rosini2015randomized,degrauwe2019influence,belin2023manually}.

\begin{table}[htbp]
  \centering
  \caption{Analysis of the outcome on mimic data}
    \begin{tabular}{c|c|c|c}
    \hline
    Method & $VAN\to WBC$     & $NE\to MBP$    & $MS\to PLT$ \\
    \hline
    Deconf.     & 6.319 & -0.279 & -1.428 \\
    S-Deconf.     & 6.814 & 6.312 & -1.428 \\
    PMMR-OR     & -0.759 & 2.055 & -3.050 \\
    PMMR-KIPW     & -3.274 & 3.040 & -2.175 \\
    PMMR-DR     & -3.886 & 1.232 & -3.509 \\
    \hline
    \end{tabular}%
  \label{tab:real}%
\end{table}%





==> chap/estimate.tex <==
\vspace{-0.2cm}
\section{Estimation}
\vspace{-0.1cm}
\label{sec.estimate}

With identified proxies $W_{S,j}$ and $Z_{S,j}$ at hand, we introduce our method to estimate the causal effect. We first solve the outcome bridge functions $h$ and treatment bridge functions $q$ from the following Fredholm integral equations, where we replace $W_{S,j}$ and $Z_{S,j}$ with $W$ and $Z$ for brevity:
\begin{equation}\label{eq.h_q}
     \mathbb{E}[Y-h(A,W) | A,Z]=0,~~~
    \mathbb{E}\left[q(A,Z)-1/p(A|W)| A,W\right]=0. 
\end{equation}
After obtaining $h$ and $q$, we employ the \cite{wuyong,colangelo2020double}


estimate $\mathbb{E}[Y|\operatorname{do}(a)]$ via the Proximal Doubly Robust (PDR) estimator: 
\begin{equation}\label{eq.DR}
  \mathbb{E}[Y\mid\operatorname{do}(a)]\approx \mathbb{E}_n[\mathbb{I}(A=a)q(a,Z)(Y-h(a,W)) + h(a,W))]. 
\end{equation}
When treatment $A$ is continuous, by \cite{colangelo2020double}, we use the kernel function instead of the indicator function, i.e. the Proximal Kernel Doubly Robust (PKDR) estimator:
\begin{equation}\label{eq.DR_kernel}
  \mathbb{E}[Y\mid\operatorname{do}(a)]\approx  \mathbb{E} _n[K_{h_{\mathrm{bw}}}\left( A-a \right) q(a,Z)(Y-h(a,W))+h(a,W))], 
\end{equation}
where $h_{\mathrm{bw}} > 0$ is the bandwidth such that $K_{h_{\mathrm{bw}}}(a_i-a) = \frac{1}{h_{\mathrm{bw}}} K\left(\frac{a_i-a}{h_{\mathrm{bw}}}\right)$. 

Intuitively, we can observe that bridge function $h$ and $q$ serve a similar role as the regression function and the propensity score in classical causal inference. In fact, suppose that $U=\emptyset$, then Eq.~\ref{eq.h_q} reduces to $h(a,W)=\mathbb{E}[Y|A=a,W]$ and $q(a,Z)=1/p(A=a|Z)$. Therefore, PKDR estimator will degenerate to doubly robust (DR) estimator.

\textbf{Nuisance function $h,q$.} To estimate causal effect, we should first estimate nuisance function $h$ and $q$. In this paper, we employ Proxy Maximum Moment Restriction (PMMR) \citep{mastouri2021proximal}, which have been shown be effective \citep{xu2021deep} in solving causal functions via kernel methods.
\begin{align}
	\min_{h\in \mathcal{H} _{\mathcal{A} \mathcal{W}}} \frac{1}{n^2}\sum_{i,j=1}^n{(y_i-h_i)(y_j-h_j)k_{ij}^{g}}+\lambda _h\left\| h \right\| _{\mathcal{H} _{\mathcal{A} \mathcal{W}}}^{2}\\
	\min_{h\in \mathcal{Q} _{\mathcal{AZ} }} \frac{1}{n^2}\sum_{i,j=1}^n{(1/p_i-q_i)(1/p_j-q_j)k_{ij}^{m}}+\lambda _q\left\| q \right\| _{\mathcal{Q} _{\mathcal{AZ}}}^{2}
\end{align}
where $k^g_{ij}:=k^g((a_i,z_i),(a_j,z_j))$, $k^m_{ij}=k^m( ( a_i,w_i),( a_j,w_j))$, $h_i:=h(a_i,w_i)$, $q_{i}:=q( a_i,z_i)$ and $p_i=p(a_i|w_i)$ . We parameterize $h$ and $q$ as reproducing kernel Hilbert space (RKHS) $\mathcal{H} _{\mathcal{A} \mathcal{W}},\mathcal{H} _{\mathcal{A} \mathcal{Z}}$ with $\left\| \cdot\right\| _{\mathcal{H} _{\mathcal{A} \mathcal{W}}},\left\| \cdot\right\| _{\mathcal{H} _{\mathcal{A} \mathcal{Z}}}$. 



==> chap/experiment_v1.tex <==
\vspace{-0.2cm}
\section{Experiments}
\vspace{-0.1cm}
\label{sec.experiment}

In this section, we evaluate our method on synthetic data and a real-world application that studies the treatment effect for sepsis disease.



\noindent\textbf{Compared baselines.} \textbf{(i) Generalized Propensity Score (GPS)} \citep{scharfstein1999adjusting} that estimated the causal effect with generalized propensity score; \textbf{(ii) Targeted Maximum Likelihood Estimation (TMLE)} \citep{van2006targeted} that used Targeted Maximum Likelihood Estimation to estimate causal effects; \textbf{(iii) POP} \citep{zhou2020promises} that used multiple outcomes and linear structural equations to estimate causal effects; \textbf{iv) Deconf. (Linear)} \citep{wang2019blessings} that estimated unobserved confounders from multiple treatments to estimate causal effects, where the outcome model is linear; \textbf{v) Deconf. (Kernel)} that the outcome model is kernel regression; \textbf{vi) P-Deconf. (Linear)} \citep{wang2021proxy} that used null proxy on the basis of \cite{wang2019blessings} to estimate causal effects, where the outcome model is linear; \textbf{vii) P-Deconf. (Kernel)} that uses kernel regression to estimate the outcome model.

\noindent\textbf{Evaluation metrics.} For the hypothesis test, we measure the precision, and recall of identified causal edges, and ${\mathrm{F}}_{1}:=2\cdot{\frac{\mathrm{precision}\cdot\mathrm{recall}}{\mathrm{precision+recall}}}$. For the causal effect estimation, we report the causal Mean Absolute Error (cMAE) across $10$ equally spaced points in $\mathrm{supp}(A):=[0,1]$: {\small $\mathrm{cMAE}:=\frac{1}{10}\sum_{i=1}^{10}|\mathbb{E}[Y^{a_i}]-\hat{\mathbb{E}}[Y^{a_i}]|$}. The truth $\mathbb{E}[Y^{a}]$ is derived through Monte Carlo simulations comprising 10,000 replicates of data generation for each $a$.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.7\textwidth]{Figure/exp_DAG.pdf}
    \caption{The causal graph over treatments (blue) and outcomes (red) of (a) synthetic data and (b) real-world data. The DAG of (b) is estimated using hypothesis testing in Sec.~\ref{sec.causal-discovery}}
    \label{fig: exp_DAG}
\end{figure}

\vspace{-0.2cm}
\subsection{Synthetic study}
\vspace{-0.1cm}


\noindent\textbf{Data generation.} We follow the DAG in Fig.~\ref{fig: exp_DAG} and following structural equations to generate data: $U\sim \operatorname{Uniform}[-1,1]$, $A_i=g_i(U)+\epsilon_i$, with $g_i$ chosen from $\{linear,tanh,sin,cos,sigmoid\}$ and $\epsilon_i\sim N(0,1)$, and $\mathbf{Y}$ is a non-linear structure, namely
$Y_1 = 2\sin(1.4A_1+2A_3^2)+0.5(A_2+A_4^2+A_5)+A_3^3+U+\epsilon_1, Y_2 = -2\cos(1.8A_2)+1.5A_4^2+U+\epsilon_{2}, Y_3 = 0.7A_3^2+1.2A_4+U+\epsilon_{3}$, and $Y_4 = 1.6e^{-A_1+1}+2.3A_5^2+U+\epsilon_{4}$ with $\{\epsilon_i\}_{i=1}^4 \sim N(0,1)$.





\emph{Independence test}: \textbf{i) Fisher} that Fisher conditional independence test; \textbf{ii) KCI} that Kernel-based conditional independence test; \textbf{iii) Chisq} that Chi-squared conditional independence test; \textbf{iv) POP} that The Promises of Parallel Outcomes. 


\noindent\textbf{Implementation details.} For hypothesis testing, we set the significant level $\alpha$ as 0.05, and the bin numbers for discretization of $A,W,Y$ as $I := |A| = 15, K := |W|= 8, L := |Y| = 5$, respectively. The asymptotic estimators in Eq.~\ref{eq.q_and_Q} are obtained by empirical probability mass functions. The sample size is set to $\{600,800,1000,1200,1400,1600\}$. To remove the effect of randomness, we repeat for $50$ replications.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.95\textwidth]{Figure/discover.pdf}
    \caption{Performance of our method and baselines under the setting of multi-treatments and multi-outcomes.}
    \label{fig:discover}
\end{figure}

\noindent\textbf{Causal discovery.} We use the proxy-based hypothesis test to recover the causal graph and report the results under different sample sizes. In Fig.~\ref{fig:discover}, we present the performance of our method and the baselines in the context of multiple treatments
and multiple outcomes. Notably, our method outperforms all others across all metrics. Firstly, it's evident that the POP method, which shares a similar multi-outcome setup, exhibits significantly lower performance due to its reliance on the unrealistic assumption of linear structural equations. Secondly, Chisq testing tends to establish connections between all edges, resulting in a high Type I error, likely stemming from the inherent nonlinearity of the structural equations. Lastly, in comparison to Fisher's and Kernel testing, our approach demonstrates superior and more stable performance, leveraging information from proxy (other treatments).



\noindent\textbf{Implementation details.} We use the PMMR method \cite{mastouri2021proximal} to solute the nuisance function $h$ and $q$. For hyperparameters for solving $h$ and $q$, please refer to the appendix
. In the PKDR estimators, we choose the Gaussian Kernel, with bandwidth $h_{\mathrm{bw}} = 1.5 \hat{\sigma}_A n^{-1/5}$ with estimated std $\hat{\sigma}_A$. We run each algorithm 20 times with sample size $600$ or $1, 200$ and calculate the mean c-MAE.
 

\noindent\textbf{Causal effect estimation.} We estimate the average causal effect of $A_3\to Y_1$, $(A_1,A_3)\to Y_1$, $A_2\to Y_2$, $(A_1,A_5)\to Y_4$ and report the results in Tab.~\ref{tab:synthetic}. As we can see, our approach show very small causal estimation bias when suitable proxies are available. In contrast, both parametric and non-parametric deconfounder algorithms display substantial errors, largely stemming from their sensitivity to arbitrary biases in effect estimation. P-deconfounder performs admirably in the presence of a null proxy but deviates significantly when no proxies exist, highlight the significance of finding appropriate proxies. For classic GPS and TMLE, their performance falters due to their failure to satisfy the conditional ignorability assumption. Additionally, POP's assumption of linear structural functions and the notion that each treatment affects all outcomes result in poor performance.





\begin{table}[htbp]
  \centering
  \caption{C-MAE of PKDR and baseline methods in Synthetic study. Each method was replicated 20 times and evaluated test values of $a\in [0,1]$ each replicate.}
   \renewcommand{\arraystretch}{1.2}
  \scalebox{0.75}{
    \begin{tabular}{c|cccc|cccc}
    \hline
    \hline
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{$A_3\rightarrow Y_1$} & \multicolumn{2}{c|}{$(A_1,A_3)\rightarrow Y_1$} & \multicolumn{2}{c|}{$A_2\rightarrow Y_2$} & \multicolumn{2}{c}{$(A_1,A_5) \rightarrow Y_4$} \\
\cline{2-9}          & 600   & 1200  & 600   & 1200  & 600   & 1200  & 600   & 1200 \\
    \hline
    GPS   & $0.97_{\pm 0.33}$ & $0.64_{\pm 0.17}$ & -       &  -     & $0.46_{\pm 0.21}$ & $0.33_{\pm 0.14}$ &  -     & - \\
    TMLE  & $0.48_{\pm 0.16}$ & $0.43_{\pm 0.16}$ & -      &   -    & $0.68_{\pm 0.28}$ & $0.42_{\pm 0.15}$ &   -    &  -\\
    POP   &  $2.64_{\pm 0.49}$     &   $2.57_{\pm 0.33}$    &  -     & -       & $2.17_{\pm 1.31}$      &   $1.52_{\pm 0.65}$    & -      &-  \\
    Deconf.(Linear) & $2.52_{\pm 0.41}$ & $2.59_{\pm 0.40}$ & $6.05_{\pm 1.58}$ & $5.81_{\pm 1.49}$ & $1.23_{\pm 0.54}$ & $1.34_{\pm 0.41}$ & $1.31_{\pm 0.35}$ & $1.16_{\pm 0.30}$ \\
    Deconf.(Kernel) & $0.60_{\pm 0.08}$ & $0.48_{\pm 0.12}$ & $4.12_{\pm 0.80}$ & $3.67_{\pm 1.10}$ & $0.35_{\pm 0.20}$ & $0.38_{\pm 0.19}$ & $0.24_{\pm 0.24}$ & $0.29_{\pm 0.25}$ \\
    P-Deconf.(Linear) & $2.52_{\pm 0.41}$ & $2.59_{\pm 0.40}$ & $6.05_{\pm 1.58}$ & $5.81_{\pm 1.49}$ & $1.08_{\pm 0.26}$ & $1.19_{\pm 0.18}$ & $1.81_{\pm 0.44}$ & $1.77_{\pm 0.27}$ \\
    P-Deconf.(Kernel) & $0.60_{\pm 0.08}$ & $0.48_{\pm 0.12}$ & $4.12_{\pm 0.80}$ & $3.67_{\pm 1.10}$ & $\mathbf{0.26_{\pm 0.16}}$ & $\mathbf{0.21_{\pm 0.14}}$ & $0.19_{\pm 0.12}$ & $\mathbf{0.20_{\pm 0.10}}$ \\
    PKDR & $\mathbf{0.28_{\pm 0.09}}$ & $\mathbf{0.27_{\pm 0.09}}$ & $\mathbf{0.49_{\pm 0.20}}$ & $\mathbf{0.48_{\pm 0.14}}$ & $0.29_{\pm 0.14}$ & $0.23_{\pm 0.09}$ & $\mathbf{0.17_{\pm 0.09}}$ & $0.22_{\pm 0.14}$ \\
    \hline
    \hline
    \end{tabular}}
  \label{tab:synthetic}%
\end{table}%





\vspace{-0.2cm}
\subsection{Treatment Effect for Sepsis Disease}
\vspace{-0.1cm}
In this section, we apply our method to the treatment effect estimation for sepsis disease.

\noindent\textbf{Data Preparation.} We consider the Medical Information Mart for Intensive Care (MIMIC III) dataset \cite{johnson2016mimic}, which consists of electronic health records from patients in the Intensive Care Unit (ICU). From MIMIC III, we extract $1165$ patients with sepsis disease. For these patients, three treatment options are recorded during their stays: Vancomycin, Morphine Sulfate, and Norepinephrine, which are commonly used to treat sepsis patients in the ICU. After receiving treatments, we record several blood count indexes, among which we consider three outcomes in this study: White blood cell count, Mean blood pressure, and Platelets.

% At the next moment, we extract three outcomes (blood count indexes): White blood cell count, Mean blood pressure, and Platelets.

\noindent\textbf{Implementation details.} For hypothesis testing, we set the significant level $\alpha$ as 0.05, and the bin numbers for discretization of $A,W,Y$ as $I := |A| = 10, K := |W|= 6, L := |Y| = 5$, respectively. The asymptotic estimators in Eq.~\ref{eq.q_and_Q} are obtained by empirical probability mass functions. For treatment effect estimation, we use the same method as synthetic data to solve $h$ and $q$ and perform causal estimation.


\noindent\textbf{Causal discovery.} Our obtained causal diagram is depicted in Fig.~\ref{fig: exp_DAG}(b). As illustrated, Vancomycin exhibits a significant causal influence on White Blood Cell Count and Platelets, which is in accordance with existing clinical research \cite{rosini2015randomized,mohammadi2017vancomycin}. Furthermore, Fig.~\ref{fig: exp_DAG} demonstrates a close association between the prescription of morphine and Mean Blood Pressure and Platelets, but it does not appear to exert a noticeable influence on White Blood Cell Counts, aligning with the known pharmacological side effects of morphine as reported in \cite{anand2004effects,degrauwe2019influence,simons2006morphine}. Additionally, we observe that Norepinephrine causally affects all blood count parameters, as also found in previous studies \cite{gader1975effect,larsson1994norepinephrine,belin2023manually}.

\noindent\textbf{Causal Effect Estimation.} We estimate the causal effect of $VAN\to WBC$, $NE\to MBP$, $MS\to PLT$. Since this is a real dataset, it is not possible to evaluate the extent of hidden confounding or to estimate the true (Oracle) treatment responses. But we can evaluate trends through prior knowledge. As we can see, vancomycin, used to control bacterial infections in patients with sepsis, initially lowered white blood cell counts and then leveled off because of its bactericidal and anti-inflammatory properties. Besides, Norepinephrine, as a vasopressor, can increase blood pressure. Also, Fig.~\ref{fig:real} shows that Morphine has a negative effect on platelet counts. Our findings are consistent with the literature studying the effects of three drugs on blood count indexes \cite{rosini2015randomized,degrauwe2019influence,belin2023manually}.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.95\textwidth]{Figure/mimic.pdf}
    \caption{Analysis of the outcome on mimic data.}
    \label{fig:real}
\end{figure}








==> chap/experiment_v2.tex <==
\vspace{-0.2cm}
\section{Experiments}
\vspace{-0.1cm}
\label{sec.experiment}

In this section, we evaluate our method on synthetic data and a real-world application that studies the treatment effect for sepsis disease.



\noindent\textbf{Compared baselines.} \textbf{(i) Generalized Propensity Score (GPS)} \citep{scharfstein1999adjusting} that estimated the causal effect with generalized propensity score; \textbf{(ii) Targeted Maximum Likelihood Estimation (TMLE)} \citep{van2006targeted} that used Targeted Maximum Likelihood Estimation to estimate causal effects; \textbf{(iii) POP} \citep{zhou2020promises} that used multiple outcomes and linear structural equations to estimate causal effects; \textbf{iv) Deconf. (Linear)} \citep{wang2019blessings} that estimated unobserved confounders from multiple treatments to estimate causal effects, where the outcome model is linear; \textbf{v) Deconf. (Kernel)} that the outcome model is kernel regression; \textbf{vi) P-Deconf. (Linear)} \citep{wang2021proxy} that used null proxy on the basis of \cite{wang2019blessings} to estimate causal effects, where the outcome model is linear; \textbf{vii) P-Deconf. (Kernel)} that uses kernel regression to estimate the outcome model.

\noindent\textbf{Evaluation metrics.} For the hypothesis test, we measure the precision, and recall of identified causal edges, and ${\mathrm{F}}_{1}:=2\cdot{\frac{\mathrm{precision}\cdot\mathrm{recall}}{\mathrm{precision+recall}}}$. For the causal effect estimation, we report the causal Mean Absolute Error (cMAE) across $10$ equally spaced points in $\mathrm{supp}(A):=[0,1]$: {\small $\mathrm{cMAE}:=\frac{1}{10}\sum_{i=1}^{10}|\mathbb{E}[Y^{a_i}]-\hat{\mathbb{E}}[Y^{a_i}]|$}. The truth $\mathbb{E}[Y^{a}]$ is derived through Monte Carlo simulations comprising 10,000 replicates of data generation for each $a$.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.7\textwidth]{Figure/exp_DAG.pdf}
    \caption{The causal graph over treatments (blue) and outcomes (red) of (a) synthetic data and (b) real-world data. The DAG of (b) is estimated using hypothesis testing in Sec.~\ref{sec.causal-discovery}}
    \label{fig: exp_DAG}
\end{figure}

\vspace{-0.2cm}
\subsection{Synthetic study}
\vspace{-0.1cm}


\noindent\textbf{Data generation.} We follow the DAG in Fig.~\ref{fig: exp_DAG} and following structural equations to generate data: $U\sim \operatorname{Uniform}[-1,1]$, $A_i=g_i(U)+\epsilon_i$, with $g_i$ chosen from $\{linear,tanh,sin,cos,sigmoid\}$ and $\epsilon_i\sim N(0,1)$, and $\mathbf{Y}$ is a non-linear structure, namely
$Y_1 = 2\sin(1.4A_1+2A_3^2)+0.5(A_2+A_4^2+A_5)+A_3^3+U+\epsilon_1, Y_2 = -2\cos(1.8A_2)+1.5A_4^2+U+\epsilon_{2}, Y_3 = 0.7A_3^2+1.2A_4+U+\epsilon_{3}$, and $Y_4 = 1.6e^{-A_1+1}+2.3A_5^2+U+\epsilon_{4}$ with $\{\epsilon_i\}_{i=1}^4 \sim N(0,1)$.


\noindent\textbf{Implementation details.} For hypothesis testing, we set the significant level $\alpha$ as 0.05, and the bin numbers for discretization of $A,W,Y$ as $I := |A| = 15, K := |W|= 8, L := |Y| = 5$, respectively. We estimate $q_y, Q$ in Eq.~\ref{eq.q_and_Q} using empirical probabilities. To remove the effect of randomness, we repeat for $50$ replications. For our causal estimator in Eq.~\ref{eq.DR_kernel}, we choose the Gaussian Kernel with bandwidth $h_{\mathrm{bw}} = 1.5\hat{\sigma}_A n^{-1/5}$ where $\hat{\sigma}_A$ is the estimated standard deviation of $A$. We run each algorithm 20 times to calculate the average cMAE.

%with sample size $600$ or $1, 200$ and calculate the mean c-MAE.
 % The sample size is set to $\{\text{600},\text{800},\text{1,000},\text{1,200}, \text{1,400},\text{1,600}\}$. 

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.95\textwidth]{Figure/discover.pdf}
    \caption{Performance of our method and baselines under the setting of multi-treatments and multi-outcomes.}
    \label{fig:discover}
\end{figure}

\noindent\textbf{Causal discovery to identify proxies.} To illustrate the effectiveness of our method, we also compare with 

We report the results in Fig.~\ref{fig:discover}. 


we present the performance of our method and the baselines in the context of multiple treatments
and multiple outcomes. Notably, our method outperforms all others across all metrics. Firstly, it's evident that the POP method, which shares a similar multi-outcome setup, exhibits significantly lower performance due to its reliance on the unrealistic assumption of linear structural equations. Secondly, Chisq testing tends to establish connections between all edges, resulting in a high Type I error, likely stemming from the inherent nonlinearity of the structural equations. Lastly, in comparison to Fisher's and Kernel testing, our approach demonstrates superior and more stable performance, leveraging information from proxy (other treatments).



\emph{Independence test}: \textbf{i) Fisher} that Fisher conditional independence test; \textbf{ii) KCI} that Kernel-based conditional independence test; \textbf{iii) Chisq} that Chi-squared conditional independence test; \textbf{iv) POP} that The Promises of Parallel Outcomes. 

\noindent\textbf{Causal effect estimation.} We estimate the average causal effect of $A_3\to Y_1$, $(A_1,A_3)\to Y_1$, $A_2\to Y_2$, $(A_1,A_5)\to Y_4$ and report the results in Tab.~\ref{tab:synthetic}. As we can see, our approach show very small causal estimation bias when suitable proxies are available. In contrast, both parametric and non-parametric deconfounder algorithms display substantial errors, largely stemming from their sensitivity to arbitrary biases in effect estimation. P-deconfounder performs admirably in the presence of a null proxy but deviates significantly when no proxies exist, highlight the significance of finding appropriate proxies. For classic GPS and TMLE, their performance falters due to their failure to satisfy the conditional ignorability assumption. Additionally, POP's assumption of linear structural functions and the notion that each treatment affects all outcomes result in poor performance.





\begin{table}[htbp]
  \centering
  \caption{C-MAE of PKDR and baseline methods in Synthetic study. Each method was replicated 20 times and evaluated test values of $a\in [0,1]$ each replicate.}
   \renewcommand{\arraystretch}{1.2}
  \scalebox{0.75}{
    \begin{tabular}{c|cccc|cccc}
    \hline
    \hline
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{$A_3\rightarrow Y_1$} & \multicolumn{2}{c|}{$(A_1,A_3)\rightarrow Y_1$} & \multicolumn{2}{c|}{$A_2\rightarrow Y_2$} & \multicolumn{2}{c}{$(A_1,A_5) \rightarrow Y_4$} \\
\cline{2-9}          & 600   & 1200  & 600   & 1200  & 600   & 1200  & 600   & 1200 \\
    \hline
    GPS   & $0.97_{\pm 0.33}$ & $0.64_{\pm 0.17}$ & -       &  -     & $0.46_{\pm 0.21}$ & $0.33_{\pm 0.14}$ &  -     & - \\
    TMLE  & $0.48_{\pm 0.16}$ & $0.43_{\pm 0.16}$ & -      &   -    & $0.68_{\pm 0.28}$ & $0.42_{\pm 0.15}$ &   -    &  -\\
    POP   &  $2.64_{\pm 0.49}$     &   $2.57_{\pm 0.33}$    &  -     & -       & $2.17_{\pm 1.31}$      &   $1.52_{\pm 0.65}$    & -      &-  \\
    Deconf.(Linear) & $2.52_{\pm 0.41}$ & $2.59_{\pm 0.40}$ & $6.05_{\pm 1.58}$ & $5.81_{\pm 1.49}$ & $1.23_{\pm 0.54}$ & $1.34_{\pm 0.41}$ & $1.31_{\pm 0.35}$ & $1.16_{\pm 0.30}$ \\
    Deconf.(Kernel) & $0.60_{\pm 0.08}$ & $0.48_{\pm 0.12}$ & $4.12_{\pm 0.80}$ & $3.67_{\pm 1.10}$ & $0.35_{\pm 0.20}$ & $0.38_{\pm 0.19}$ & $0.24_{\pm 0.24}$ & $0.29_{\pm 0.25}$ \\
    P-Deconf.(Linear) & $2.52_{\pm 0.41}$ & $2.59_{\pm 0.40}$ & $6.05_{\pm 1.58}$ & $5.81_{\pm 1.49}$ & $1.08_{\pm 0.26}$ & $1.19_{\pm 0.18}$ & $1.81_{\pm 0.44}$ & $1.77_{\pm 0.27}$ \\
    P-Deconf.(Kernel) & $0.60_{\pm 0.08}$ & $0.48_{\pm 0.12}$ & $4.12_{\pm 0.80}$ & $3.67_{\pm 1.10}$ & $\mathbf{0.26_{\pm 0.16}}$ & $\mathbf{0.21_{\pm 0.14}}$ & $0.19_{\pm 0.12}$ & $\mathbf{0.20_{\pm 0.10}}$ \\
    PKDR & $\mathbf{0.28_{\pm 0.09}}$ & $\mathbf{0.27_{\pm 0.09}}$ & $\mathbf{0.49_{\pm 0.20}}$ & $\mathbf{0.48_{\pm 0.14}}$ & $0.29_{\pm 0.14}$ & $0.23_{\pm 0.09}$ & $\mathbf{0.17_{\pm 0.09}}$ & $0.22_{\pm 0.14}$ \\
    \hline
    \hline
    \end{tabular}}
  \label{tab:synthetic}%
\end{table}%


\vspace{-0.2cm}
\subsection{Treatment Effect for Sepsis Disease}
\vspace{-0.1cm}
In this section, we apply our method to the treatment effect estimation for sepsis disease.

\noindent\textbf{Data Preparation.} We consider the Medical Information Mart for Intensive Care (MIMIC III) dataset \cite{johnson2016mimic}, which consists of electronic health records from patients in the Intensive Care Unit (ICU). From MIMIC III, we extract $1165$ patients with sepsis disease. For these patients, three treatment options are recorded during their stays: Vancomycin, Morphine Sulfate, and Norepinephrine, which are commonly used to treat sepsis patients in the ICU. After receiving treatments, we record several blood count indexes, among which we consider three outcomes in this study: White blood cell count, Mean blood pressure, and Platelets.


\noindent\textbf{Implementation details.} For hypothesis testing, we set the significant level $\alpha$ as 0.05, and the bin numbers for discretization of $A,W,Y$ as $I := |A| = 10, K := |W|= 6, L := |Y| = 5$, respectively. The asymptotic estimators in Eq.~\ref{eq.q_and_Q} are obtained by empirical probability mass functions. For treatment effect estimation, we use the same method as synthetic data to solve $h$ and $q$ and perform causal estimation.


\noindent\textbf{Causal discovery.} Our obtained causal diagram is depicted in Fig.~\ref{fig: exp_DAG}(b). As illustrated, Vancomycin exhibits a significant causal influence on White Blood Cell Count and Platelets, which is in accordance with existing clinical research \cite{rosini2015randomized,mohammadi2017vancomycin}. Furthermore, Fig.~\ref{fig: exp_DAG} demonstrates a close association between the prescription of morphine and Mean Blood Pressure and Platelets, but it does not appear to exert a noticeable influence on White Blood Cell Counts, aligning with the known pharmacological side effects of morphine as reported in \cite{anand2004effects,degrauwe2019influence,simons2006morphine}. Additionally, we observe that Norepinephrine causally affects all blood count parameters, as also found in previous studies \cite{gader1975effect,larsson1994norepinephrine,belin2023manually}.

\noindent\textbf{Causal Effect Estimation.} We estimate the causal effect of $VAN\to WBC$, $NE\to MBP$, $MS\to PLT$. Since this is a real dataset, it is not possible to evaluate the extent of hidden confounding or to estimate the true (Oracle) treatment responses. But we can evaluate trends through prior knowledge. As we can see, vancomycin, used to control bacterial infections in patients with sepsis, initially lowered white blood cell counts and then leveled off because of its bactericidal and anti-inflammatory properties. Besides, Norepinephrine, as a vasopressor, can increase blood pressure. Also, Fig.~\ref{fig:real} shows that Morphine has a negative effect on platelet counts. Our findings are consistent with the literature studying the effects of three drugs on blood count indexes \cite{rosini2015randomized,degrauwe2019influence,belin2023manually}.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.95\textwidth]{Figure/mimic.pdf}
    \caption{Analysis of the outcome on mimic data.}
    \label{fig:real}
\end{figure}




==> chap/introduction.tex <==
\vspace{-0.2cm}
\section{Introduction}
\vspace{-0.1cm}
\label{sec.intro}

Estimating average causal effects from observed data is an important problem in many areas, such as social sciences, biological sciences, and economics, \emph{etc}. However, the presence of unobserved confounders makes the result unreliable, since it can introduce bias into the estimation. To tackle this problem, existing works relied on additional measurements, such as instrumental variables \cite{pokropek2016introduction}, proxy variables \cite{miao2018identifying} and additional treatments \cite{wang2019blessings}.




there is rising attention \cite{miao2018identifying, tchetgen2020introduction,cui2020semiparametric} toward proximal causal learning, due to its ability to account for unmeasured counfounders through two confounding proxy variables: a treatment-inducing proxy and an outcome-inducing proxy, which are respectively independent to the outcome and the treatment given the unobserved confounders. With such suitable proxy variables, \cite{miao2018identifying,cui2020semiparametric} showed that the true causal effect can be identified with estimated nuisance parameters. Further, 

\cite{miao2022identifying,wang2021proxy} associated the proxy variables with \textit{multiple treatments}, which allow us to identify a type of proxies, \emph{i.e.}, other treatments. However, this approach required the existence of an additional null proxy that has no effect on the outcome, which may not always be satisfied for a fixed outcome. Therefore, we consider a natural extension from a single outcome to multiple outcomes under the \textit{multiple treatments} setting, which allow us to leverage other outcomes to act as null proxies. This scenario, which is commonly referred to as \emph{multiple (treatment, outcome)-effects estimation}, can widely exist in many real-world applications such as the clinical decision support system. To illustrate, consider the Intensive Care Unit (ICU) scenario with sepsis disease \cite{johnson2016mimic} as a motivating example. In this setting, healthcare providers may monitor various parameters, such as complete blood counts (CBC) \cite{kutlucan2016predictive} (\emph{e.g}., White blood cell count, Mean blood pressure, and Platelets), to evaluate the effectiveness of therapeutic treatments (such as Norepinephrine, Morphine Sulfate, and Vancomycin).
% As a result, healthcare providers require knowledge of the therapeutic effect of each treatment for each outcome to ensure that all indicators are within normal limits.

Note that a recent study \cite{zhou2020promises} has demonstrated that nonparametric identifiability under the assumption of conditional independence among at least three parallel outcomes. However, this relied on the \emph{no qualitative $U$-$A$ interaction} assumption, which may not hold when the outcome model of $Y|U,A$ is complex. Furthermore, their approach was limited to a single treatment, which may not adequately address scenarios where multiple treatments are under investigation, as in the ICU scenario mentioned earlier. \textbf{In contrast}, our methods additionally leverage multiple treatments, which allow us to leverage proxies for identification.


In this paper, we consider the scenario where multiple treatments and outcomes are simultaneously accessible. We first show the existence of the treatment-inducing and outcome-inducing proxies for each treatment effect, as long as the bipartite graph between treatments and outcomes is not overly dense. It can naturally hold since, as we consider the ICU example in which not all therapeutic treatments are effective to any specific indicator. To identify such proxies, we employ hypothesis testing for edges between each treatment and outcome, via a proper discretization of treatments. With such identified proxies, we employ the proximal doubly robust estimator in estimating the treatment effect. The utility and effectiveness of our methods are demonstrated on a synthetic dataset and Medical Information Mart for Intensive Care (MIMIC III) \cite{johnson2016mimic}.

% in scenarios with multiple treatments and multiple outcomes, some outcomes may be only associated with a few treatments.

 
\textbf{Contributions.} To summarize, our contributions are: 
\begin{enumerate}[topsep=0.1ex,leftmargin=*]
    \item We consider a new scenario in which multiple treatments and outcomes are simultaneously accessible. Particularly, the multiple outcomes provided can enable us to identify the proxies for causal identification. 
    \item We employ hypothesis testing via a proper discretization of treatments to identify proxies. 
    \item We demonstrate the utility of our methods on both synthetic and real-world data. 
\end{enumerate}


